Online Stochastic Matching with Unknown Arrival Order: Beating $0.5$ against the Online Optimum

We study the online stochastic matching problem. Against the offline benchmark, Feldman, Gravin, and Lucier (SODA 2015) designed an optimal $0.5$-competitive algorithm. A recent line of work, initiated by Papadimitriou, Pollner, Saberi, and Wajc (MOR 2024), focuses on designing approximation algorithms against the online optimum. The online benchmark allows positive results surpassing the $0.5$ ratio. In this work, adapting the order-competitive analysis by Ezra, Feldman, Gravin, and Tang (SODA 2023), we design a $0.5+\Omega(1)$ order-competitive algorithm against the online benchmark with unknown arrival order. Our algorithm is significantly different from existing ones, as the known arrival order is crucial to the previous approximation algorithms.

==> large_7.3.tex <==
\subsection{Proof of \Cref{lma:largenorm}}

We first construct solution $z$ via the following process:
\begin{itemize}
    \item Initiate $\tilde{b}= \tildyl$.
    \item For each $t$ such that $q_t(\tilde{b}) > q_t(\tildxl)$, arbitrarily reduce the value of $\tilde{b}_{it}$ until $q_t(\tilde{b}) = q_t(\tildxl)$ is satisfied.
\end{itemize}

The generated $z$ satisfies $q_t(\tilde{b}) \leq q_t(\tildxl)$ for every $t \in V$. Let solution $\bar{b} = \tildxl + \tildyl - \tilde{b}$. Then, solution $\bar{b}$ is feasible, because we have  $q_i(\bar{b}) \leq q_i(\tildxl) + q_i(\tildyl) \leq \probfr + \epsphilo^{1/4}$ for every $i \in U$, and $q_t(\bar{b}) \leq q_t(\tildyl) \leq p_t$ for every $t \in V$. Consider the following two cases:

\paragraph{Case 1: $\lp(\bar{b}) \ge \frac{0.5+\eps}{1-\probfr - \epsphilo^{1/4}}$.} Note that $q_i(\bar{b}) \leq 2 \cdot \frac{q_i(\tildxl) + q_i(\tildyl)}{2} \leq \probfr + \epsphilo^{1/4}$. Then, if $\lp(\bar{b}) \ge \frac{0.5+\eps}{1-\probfr - \epsphilo^{1/4}}$, there must be
\[
\stlb(\bar{b}) ~\geq~ \sum_{i \in U} (1 - \probfr - \epsphilo^{1/4}) \cdot \lp_i(\bar{b}) ~\geq~ (1 - \probfr - \epsphilo^{1/4}) \cdot \lp(\bar{b}) ~\geq~ 0.5 + \eps.
\]
Therefore, $\bar{b}$ would be the desired solution for \Cref{lma:largenorm} when  $\lp(\bar{b}) \ge \frac{0.5+\eps}{1-\probfr - \epsphilo^{1/4}}$. 


\paragraph{Case 2: $\lp(\bar{b}) < \frac{0.5+\eps}{1-\probfr - \epsphilo^{1/4}}$.} In this case, consider the solution 
\[
b = (1 - \epsphilo^{1/4}) \cdot (\tildx - \tildxl) + \tilde{b}.
\]
Solution $b$ is feasible because for $i \in U$, we have 
\[
q_i(b) ~\leq~ (1 - \epsphilo^{1/4}) \cdot q_i(\tildx) + q_i(\tilde{b}) ~\leq~ 1 - \epsphilo^{1/4} + q_i(\tildyl) ~\leq~ 1,
\]
On the other hand, for $t \in V$, we have
\[
q_t(b) ~=~ (1 - \epsphilo^{1/4}) \cdot (q_t(\tildx) - q_t(\tildxl)) + q_t(\tilde{b}) ~\leq~ q_t(\tildx) - q_t(\tildxl) + q_t(\tildxl) ~\leq~ p_t.
\]
Therefore, solution $b$ is feasible.


Now consider the value of $\stlb(b)$. Let $U_3 = \{i: 2\lp_i(\tildx) \leq \lp_i(\tildy)\}$ and $U_4 = \{i: 2\lp_i(\tildx) > \lp_i(\tildy)\}$. For $i \in U_3$, a feasible baseline algorithm would be setting a threshold $\lp_i(\tildy)$. Since $\tildx_{it} - \tildxl_{it} > 0$ only when $w_{it} < 2\lp_i(\tildx) \leq \lp_i(\tildy)$, setting the threshold to be $\lp_i(\tildy)$ could only take values when $\tilde{b}_{it} > 0$. Note that $q_i(\tilde{b}) \leq q_i(\tildyl) \leq \epsphilo^{1/4}$, so setting the threshold to be $\lp_i(\tildy)$ gets at least $(1 - \epsphilo^{1/4}) \cdot \lp_i(\tilde{b})$. Therefore,
\begin{align}
    \stlb(b) ~\geq&~ \sum_{i \in U_3} (1 - \epsphilo^{1/4}) \lp_i(\tilde{b}) + \sum_{i \in U_4} \frac{1}{2} \cdot \lp_i(b) \notag \\
    ~\geq&~ \sum_{i \in U_3} \frac{1}{2}\cdot \lp_i(b)  + \sum_{i \in U_3} \frac{1}{2} \cdot \big( \lp_i(\tilde{b}) + \lp_i(\tildxl) - \lp_i(\tildx)\big) + \sum_{i \in U_4} \frac{1}{2} \cdot \lp_i(b) - \epsphilo^{1/4} \notag \\
    ~\geq&~ \frac{1}{2} \lp(b) - \epsphilo^{1/4} + \frac{1}{2} \sum_{i \in U_3} \big(\lp_i(\tildyl) - (0.5 + 4\probfr) \lp_i(\tildx)\big) + \frac{1}{2} \sum_{i \in U_3} \big(\lp_i(\tilde{b}) - \lp_i(\tildyl)\big),\label{eq:largenorm1}
\end{align}
where the second inequality uses the fact that $\tilde{b} = \frac{1}{2} b + \frac{1}{2} \tilde{b} - \frac{1 - \epsphilo^{1/4}}{2} \cdot (\tildx - \tildxl)$, and the third inequality uses the fact that $\lp_i(\tildxl) \geq (0.5-4\probfr) \cdot \lp_i(\tildx)$.

We further bound the last two terms of \eqref{eq:largenorm1}. For the third term, we have
\begin{align}
    \sum_{i \in U_3} \big(\lp_i(\tildyl) - (0.5 + 4\probfr) \lp_i(\tildx)\big) ~&\geq~ \sum_{i \in U_3} \big((0.5 - 3\epsphilo^{1/4})\lp_i(\tildy) - (0.5 + 4\probfr) \lp_i(\tildx)\big)\notag  \\
    ~&\geq~ \frac{1}{2} \sum_{i \in U_3} \big(\lp_i(\tildy) - \lp_i(\tildx) \big) - 3\epsphilo^{1/4} - 4\probfr \notag \\
    ~&\geq~ \frac{1}{2}\yifanb - 3\epsphilo^{1/4} - 4\probfr, \label{eq:largenorm2}
\end{align}
where the last inequality follows from the assumption in \Cref{lma:largenorm}. For the last term of \eqref{eq:largenorm1}, we have
\begin{align}
    \sum_{i \in U_3} \big(\lp_i(\tilde{b}) - \lp_i(\tildyl)\big) ~&\geq~ \sum_{i \in U} \big(\lp_i(\tilde{b}) - \lp_i(\tildyl)\big) \notag \\
    ~&=~ \lp(\tilde{b}) - \lp(\tildyl) ~=~ \lp(\tildxl) - \lp(\bar{b}) \label{eq:largenorm3}
\end{align}
Now apply \eqref{eq:largenorm2} and \eqref{eq:largenorm3} back to \eqref{eq:largenorm1}, we have
\begin{align*}
    \stlb(b) ~\geq&~~ \frac{1}{2} \lp(b) - \epsphilo^{1/4} + \frac{1}{4} \yifanb - \frac32 \epsphilo^{1/4} - 2\probfr + \frac{1}{2} \lp(\tildxl) - \frac{1}{2} \lp(\bar{b}) \\
    ~=&~~ \frac{1}{2} (1 - \epsphilo^{1/4}) \cdot \big(\lp(\tildx) - \lp(\tildxl)\big) + \frac{1}{2}\big( \lp(\tildxl) + \lp(\tildyl) - \lp(\bar{b}) \big) \\
    &+ \frac{1}{2} \lp(\tildxl) - \frac{1}{2} \lp(\bar{b}) + \frac{1}{4} \yifanb - \frac52 \epsphilo^{1/4} - 2\probfr \\
    ~\geq&~~ \frac{1}{2} \big(\lp(\tildx) + \lp(\tildxl) + \lp(\tildyl) - 2\lp(\bar{b})\big)  + \frac{1}{4} \yifanb - 3 \epsphilo^{1/4} - 2\probfr ,
\end{align*}
where the second line uses the definition of $b$ and the fact that $\tilde{b}= \tildxl + \tildyl - \bar{b}$.
Finally, applying the bounds for $\lp(\tildx), \lp(\tildxl), \lp(\tildyl)$ from \yifan{There is no more lemma. Say something else.} \Cref{lma:frdtx} and \Cref{lma:frdty} and the assumption $\lp(\bar{b}) < \frac{0.5 + \eps}{1 - \probfr - \epsphilo^{1/4}}$ to the above inequality gives $\stlb(b) \geq 0.5 + \eps_b$, where
\begin{align*}
    \eps_b ~&=~ \frac{\yifanb}{4} - \frac{\eps_x + 0.5 \eps_x + \eps_l + 3.5 \epsphilo^{1/4}}{2} - \left(\frac{0.5 + \eps}{1 - \probfr - 3\epsphilo^{3/8}} - 0.5\right) - \frac{9\epsphilo^{3/8}}{2} - \eps_l \\
    ~&\geq~\frac{\yifanb}{4} - \frac{3\eps_x}{4} - \frac{3\eps_l}{2} - \probfr - \frac{7\epsphilo^{1/4}}{4} - \frac{15\epsphilo^{3/8}}{2} - 2\eps.
\end{align*}

\enze{
\begin{align*}
    \eps_b 
    ~&\geq~\frac{1}{4}\yifanb - \frac12 (3.5 \epsphilo^{1/4} + 5.5\probfr) - (\eps +\probfr + \epsphilo^{1/4}) - 3 \epsphilo^{1/4} - 2\probfr \\
    ~&=~\frac{1}{4}\yifanb - \frac{23}{4}\epsphilo^{1/4} - \frac{23}{4}\probfr - \eps\\
    ~&\geq~\frac{1}{4}\yifanb - 6\epsphilo^{1/4} -6\eps^{1/4}\\
\end{align*}
}

\enze{first inequality holds when $\eps + \probfr + \epsphilo^{1/4} \leq \frac12$ and second inequality holds when $\eps \leq 10^{-4}$}


==> slackness_bak.tex <==
\section{Main Algorithm and Proof Overview}
% \section{Preprocessing and the Slackness LP}

We now present our main algorithm for proving Theorem~\ref{thm:main}. Starting from this section, for the ease of notation, we normalize
$\lpexante$ to be $1$.

Our algorithm consists of three parameters $\eps, \epsphilo, \epsslack$, that are constants to be optimized.
Our target is to have a $(0.5+\eps)$ order-competitive ratio. The meaning of the other two parameters shall be clear soon.
% and we are going to choose the parameters at the end of the section.

\paragraph{Step 1:}
As the first step, we solve the ex-ante relaxation and check if the following inequality holds:
\begin{equation}
\label{eqn:checkbase}
\stlb(x^*) \ge 0.5+\eps~.
\end{equation}
Recall that $\lpexante$ is renormalized as $1$. Therefore, if \eqref{eqn:checkbase} is satisfied, the baseline algorithm $\algbase(x^*)$ is at least $(0.5+\eps)$-competitive and we simply run this algorithm. Observe that the quantity $\stlb(x^*)$ can be efficiently calculated, and hence, this procedure is efficient.

\paragraph{Step 2:}
From now on, we assume that
\begin{equation}
\label{eqn:basenot}
\stlb(x^*) < 0.5+\eps~.
\end{equation}

Applying Lemma~\ref{lma:frdt} to $x^*$ and $\alpha=2$, we calculate $\tilde x$ and $\tilde x^L$ with the following properties. 
% For notation simplicity, let 
% \[
% L \eqdef \{(i,t): \wit \ge 2\cdot\lp_i(x)\}~.
% \]
\begin{itemize}
    \item $\lp(\tilde x) \ge (1-\eps^{1/4}) $~;
    \item $q_i(\tildxl) = \sum_t \tilde x_{it}^L \le \probfr$ for every $i \in U$, where we define $\probfr ~:=~ \eps^{1/4}$.
    \item $(0.5 - 4 \eps^{\nicefrac{1}{4}}) \cdot \lp_i(\tilde{x}) \leq \lp_i(\tilde x^L) \leq (0.5 + \eps^{\nicefrac{1}{4}} ) \cdot \lp_i(\tilde x)$, which implies $(0.5 - 4.5\eps^{1/4}) \leq \lp(\tildxl) \leq 0.5 + \eps^{1/4}$.
\end{itemize}
For the rest of the paper, we use $L$ to denote the edge set 
\begin{equation}
L \eqdef \{ (i,t) \in E: \wit \ge 2 \cdot \lp_i(\tilde x)\}~.
\end{equation}
This notation is consistent with $\tilde x^L$ as it can be interpreted as $\tilde x_{it}^L = \tilde x_{it} \cdot \one[(i,t) \in L]$.

Each edge in $L$ is referred to as the ``free'' edges of our instance, while each $(i, t) \in E \setminus L$ is considered a ``deterministic'' edge. These two concepts correspond to the ``free'' and ``deterministic'' vertices discussed in Section~\ref{sec:warmup}. As we extend the vertex-weighted setting from Section~\ref{sec:warmup} to the edge-weighted setting, the definitions of ``free'' and ``deterministic'' vertices are similarly generalized to ``free'' and ``deterministic'' edges.

% For notation simplicity, we use $L_i$ to denote $L_i(x^*)$, and $L$ to denote the union of $L_i$'s.

\paragraph{Step 3:}
In step 1, we checked whether $\stlb(x^*)$ is large enough so that the baseline algorithm $\algbase(x^*)$ can achieve a competitive ratio strictly greater than $0.5$. 
A natural extension is to examine the following statement:
\begin{equation}
\label{eqn:check}	
\exists x, \quad \stlb(x) > 0.5+\eps~.
\end{equation}
If so, we could simply apply the baseline algorithm with the corresponding $x$; else, it should provide more information of the instance. 
Informally, the instance should satisfy an appropriate notion of uniqueness (assumptions 5 of Section~\ref{sec:warmup}) when \eqref{eqn:check} fails.
Unfortunately, it is computationally inefficient to verify \eqref{eqn:check}, since $\stlb(x)$ is generally non-concave in $x$. To resolve this issue, we introduce the following \emph{slackness LP}. 
% \yifan{Should it be LP\_exante below?} \zhihao{Why? This is the slackness lp.}
% \yifan{I mean the last notation in second line}
% \zhihao{where $\epsphilo$ is a parameter to be optimized.}
% to examine the slackness of the optimal solution of the ex-ante relaxation. 
\begin{align*}
\max_{y}: \quad & \sum_{(i,t) \in E} \wit \cdot \tilde x^L_{it} \cdot \left(1 - \frac{\yit}{p_t} \right) + \sum_{(i,t) \in L} \wit \cdot \yit \cdot \left(1 - \frac{\tilde x^L_{it}}{p_t} \right) \tag{$\lpslack$} \\
\text{subject to:} \quad & \sum_{(i,t) \in E} \wit \cdot \yit \ge (1-\epsphilo) \cdot \lpexante \notag \\
& \sum_{i} \yit \le p_t & \forall t \in R \notag \\
& \sum_{t} \yit \le 1 & \forall i \in L \notag
\end{align*}

Intuitively speaking, the slackness LP verifies if there is an $\epsphilo$-approximately optimal solution $y$ with a large distance from $\tilde x$ on larges edges $L$, where $\epsphilo$ is the second parameter of our algorithm. Note that
\[
\lpslack ~\geq~ \sum_{(i,t) \in L} \wit \cdot (\tildxl_{it} - \yit)^+ + \sum_{(i,t) \in L} \wit \cdot (\yit - \tildxl_{it})^+ ~=~ \sum_{(i,t) \in L} \wit \cdot |\tildxl_{it} - \yit|,
\]
where notation $r^+$ represents $\max\{r, 0\}$. Therefore, when $\lpslack$ is small, it implies either $\lp(y^*)$ is bounded by $1 - \epsphilo$, or the decisions made by $y^*$ and $\tildx$ on free edges are almost the same, where we recall $y^*$ is the corresponding solution of $\lpexante$ for the optimal online algorithm.


Motivated by the above observation, depending on the value of $\lpslack$ and using $\epsslack$ as the cutting point, we branches with two different algorithms. The exact use of the slackness LP shall be highlighted in the next two sections.


\paragraph{Modeling the assumptions in Section~\ref{sec:warmup}.} With the introduction of $\lpslack$, all five assumptions from Section~\ref{sec:warmup} are addressed in this section. Before continuing to present the branched algorithm, we provide a brief summary of how these assumptions are modeled in our main algorithm.
\begin{itemize}
    \item Assumption 1 (free/deterministic vertices), Assumption 2 (vertex-weighted), and Assumption 4 (balance between free and deterministic parts): These assumptions are addressed by our free-deterministic decomposition. When applying \Cref{lma:frdt} to the solution $x^*$, the free/deterministic vertices assumption is generalized to free/deterministic edges (edge sets $L$ and $E \setminus L$), and the vertex-weighted assumption is extended to edge weights. The balance between the free and deterministic parts is ensured by \Cref{lma:frdt}.
    \item Assumption 3 ($\philo = \lpexante$): This is captured in $\lpslack$, where we only consider the solution $y$ that satisfies $\lp(y) \geq 1 - \epsphilo$. If $\lp(y^*) < 1 - \epsphilo$, we will show later in \Cref{cor:small_slack} that running $\algbase(x^*)$ in this case is sufficient.
    \item Assumption 5 (uniqueness): We extend the uniqueness assumption by requiring that the solution $y^*$ is unique for free edges. This holds when $\lpslack$ is bounded by $\epsslack$, as the weighted difference between $\tildx$ and $y^*$ on free edges is limited by $\epsslack$ (see the discussion above). When $\lpslack > \epsslack$, we will demonstrate below in \Cref{thm:large_slack} that a separated algorithm can identify a solution $z$ such that $\stlb(z)$ is at least $0.5 + \eps$.
\end{itemize}


%After introducing $\lpslack$, all 5 assumptions in Section~\ref{sec:warmup} are covered by our general algorithm. Before  

\medskip

Now, we continue to discuss our branched algorithm, which is based on whether $\lpslack \leq \epsslack$.
\paragraph{Step 3a, Large Slackness.}
 When $\lpslack$ is large (at least $\epsslack$), we show the existence of a good baseline algorithm, i.e., we prove \eqref{eqn:check}. To be specific, we give the following \Cref{thm:large_slack}.
\begin{restatable}{Theorem}{thmlargeslack}
\label{thm:large_slack}
If $\lpslack \ge \epsslack$,   there exists $z \in P$ with $\stlb(z) \ge 0.5+ \eps$ when $10^{-4} \geq \epsphilo \geq 3\eps$ and $\epsslack \ge 150(\eps^{1/4}+\epsphilo^{1/4})$ are both satisfied.

Furthermore, the solution $z$ can be computed efficiently.
\end{restatable}

Let $y^o$ be the optimal solution of $\lpslack$. Intuitively, when $\lpslack$ is large, $\tildx$ and $y^o$ are both high-value solutions, but make different decisions on edge set $L$. We make use of this difference to properly merge solutions $\tildx$ and $y^o$ into $z$, and show that $\stlb(z)$ is sufficiently large. The detailed proof of \Cref{thm:large_slack} is provided in Section~\ref{sec:large_slackness}.



\paragraph{Step 3b, Small Slackness.}
The challenging case is when $\lpslack$ is small (at most $\epsslack$). Indeed, this is the only place where our algorithm adapts to the arrival order. And we are now in a similar situation as in the warm-up section. 
We generalize the algorithm of Section~\ref{sec:warmup} so that it works well when $\philo$ is sufficiently close to $\lpexante = 1$. The proof of the following theorem is provided in Section~\ref{sec:small_slackness}.


\begin{restatable}{Theorem}{thmsmallslack}
\label{thm:small_slack}
If $\lpslack < \epsslack$, there exists an order-unaware algorithm $\alg$ that achieves an expected reward of $0.625 - 1.5 \epsslack^{1/3} - \epsphilo - 6\eps^{1/4} - \epsslack$, as long as the optimal order-aware algorithm is $\epsphilo$-approximate to the ex-ante optimum, i.e., when $\philo \ge 1-\epsphilo$.
\end{restatable}
We defer the detailed proof of \Cref{thm:small_slack} to Section~\ref{sec:small_slackness}, and first show how to use \Cref{thm:small_slack} to give a $0.5 + \eps$ order-competitive algorithm. Recall that \Cref{thm:large_slack} assumes $\epsslack \geq \Omega(\eps^{1/4} + \epsphilo^{1/4})$. With this extra assumption, we give the following corollary:



\begin{Corollary}
\label{cor:small_slack}
If $\lpslack < \epsslack$, while we have $10^{-4} \geq \epsslack \geq 150(\eps^{1/4} + \epsphilo^{1/4})$, there exists an order-unaware algorithm with order-competitive ratio $0.5 + (\nicefrac{1}{16}-\epsslack^{\nicefrac{1}{3}}) \cdot \epsphilo$. 
\end{Corollary}

\begin{proof}
Let 
\[
c =  0.625 - 1.5 \epsslack^{1/3} - \epsphilo - 6\eps^{1/4} - \epsslack - 0.5 ~\geq~ 0.125 - 2\epsslack^{1/3},
\]
where the second inequality holds when  $10^{-4} \geq \epsslack \geq 150(\eps^{1/4} + \epsphilo^{1/4})$ is satisfied. We run the algorithm $\alg$ from Theorem~\ref{thm:small_slack} with probability $\delta_{\alg}$, and $\algbase(x^*)$ with probability $1-\delta_{\alg}$. This is a randomized order-unaware algorithm. Note that
\begin{itemize}
\item If $\philo < 1-\epsphilo$, the expected reward of our algorithm is at least
\[
(1-\delta_{\alg}) \cdot 0.5  ~\ge~ 0.5 \cdot \frac{1-\delta_{\alg}}{1-\epsphilo} \cdot \philo~.
\]
\item If $\philo \ge 1-\epsphilo$, the expected reward of our algorithm is at least
\[
\delta_{\alg} \cdot (0.5 + c)  + (1-\delta_{\alg}) \cdot 0.5  = 0.5 + c \cdot \delta_{\alg} ~\geq~ (0.5 + c \cdot \delta_{\alg}) \cdot \philo
\]
\end{itemize}


By setting $\delta_{\alg} = \frac{\epsphilo}{1+2c(1-\epsphilo)} $, the randomized algorithm guarantees an order competitive ratio of 
\[
\Gamma = 0.5 + \frac{c \cdot \epsphilo}{1+2c \cdot (1-\epsphilo)} ~\geq~ 0.5 + \left (\frac{1}{16} - \epsslack^{1/3} \right) \cdot \epsphilo,
\]
where we use $c \geq 0.125 - 2\epsslack^{1/3}$ and $1 + 2c\cdot (1 - \epsphilo) \leq 1 + 2\cdot 0.125 < 2$ in the last inequality.
\end{proof}


%the instance does not satisfy the uniqueness assumption (as made in the warm-up section). The exact use of the slackness LP shall be highlighted in the next two sections.

\subsection{Proof of Theorem~\ref{thm:main}}
\label{sec:ratio}
Finally, we prove \Cref{thm:main} by combining \Cref{thm:large_slack} and \Cref{cor:small_slack}.

We set $\eps = 10^{-27}$, $\epsphilo = 256 \cdot 10^{-27}$, and $\epsslack = 10^{-6} \geq 150(\eps^{1/4} + \epsphilo^{1/4}) = 7.5 \cdot 10^{-7}$. Since the condition for \Cref{thm:large_slack} is satisfied, we have a feasible solution $z$ of $\lpexante$, such that $\algbase(z) \geq \stlb(z) \geq 0.5 + \eps$, which implies a $(0.5 + \eps)$ order-competitive algorithm when $\lpslack \geq \epsslack$. On the other hand, when $\lpslack < \epsslack$, \Cref{cor:small_slack} guarantees the order competitive ratio is at least $0.5 + (\frac{1}{16} - \epsslack^{1/3}) \cdot \epsphilo \geq 0.5 + \eps$. Therefore, we have a $(0.5 + \eps)$ order-competitive algorithm in both cases, which proves \Cref{thm:main}.




\paragraph{Why is $\eps$ so small.} We remark that the constants in our analysis are not fully optimized. We believe the value of $\eps$ can be improved to approximately $10^{-20}$ by providing a more careful analysis. However, from \Cref{thm:small_slack}, we require $O(\epsslack^{1/3}) \leq 0.125$ to achieve a competitive ratio greater than $0.5$, and \Cref{thm:large_slack} implies that $\epsslack \geq \Omega(\eps^{1/4})$. Consequently, the maximum feasible value for $\eps$ is at most $(0.125)^{12}$, with an additional significant constant loss from \Cref{thm:large_slack}. We leave it as an open question whether an order-unaware algorithm can achieve a competitive ratio significantly greater than $0.5 + 10^{-27}$, perhaps around $0.51$.

==> smallslack_bak.tex <==
\section{Small slackness}
\label{sec:small_slackness}

In this section, we study the case when the slackness of instance is small and prove the following \Cref{thm:lp_uniq_small}:

\yifan{This thm should go to preprocessing.}


\begin{Theorem}
\label{thm:lp_uniq_small}
    If $\philo \ge (1-\epsphilo) \cdot \lpexante$ and $\lpcore \le \epsslack$, there exists an order-unaware algorithm that collects an expected reward of $TBD$.
\end{Theorem}

\subsection{Our Algorithm}
\yifan{Give a name?}

Our algorithm consists of two components: 1) an online algorithm that maintains a fractional solution $\{\xit\}$ of the instance; 2) an online rounding algorithm applying to our fractional solution. 

The formal description of our algorithm is provided below. It is a generalization of the algorithm described in Section~\ref{sec:warmup}.
\begin{tcolorbox}[title=Algorithm when $\lpcore$ is small] 
Initialization:
\begin{enumerate}[(1)]
    \item Initiate $\xit = \tildxl_{it}$ for every $(i,t) \in E$. 
    \item Initiate $t_i = \infty$ for every $i \in U$. If $t \le t_i$, we say vertex $\ui$ is in the first stage, else we say $\ui$ is in the second stage. Initially, all offline vertices are in the first stage.
    \item For notation simplicity, we introduce a dummy offline vertex $0$ with $w_{0t} = 0$ for every $t \in V$, and let 
    \[
    x_{0t} = p_t - \sum_{i} \xit~.
    \]
    During the algorithm, condition $q_t(x) = p_t$ is always satisfied.
\end{enumerate}
\vspace{0.5cm}

Upon the arrival of $\vt$:
\begin{enumerate}[Step 1:]
    \item Let $\vt$ propose to $\ui$ with probability $\frac{\xit}{p_t}$ if $\vt$ is realized.
    \item If $\ui$ receives a proposal from $\vt$:
        %\begin{itemize}
         %   \item if $t \le t_i$, greedily select the edge $(i,t)$ if $\ui$ is unmatched at time $t$;
            %\item if $t > t_i$, select the edge $(i,t)$ if $\ui$ is unmatched at time $t$ with probability:
            %\[
            %\frac{1}{2 (1 - \nicefrac{1}{2} \cdot \sum_{t_i < s < t} \xit[s])}~.
            %\]
        %\end{itemize}
    \yifan{
        \begin{itemize}
            \item if $t_i = \infty$, greedily select the edge $(i,t)$ if $\ui$ is unmatched at time $t$;
            \item Otherwise, select the edge $(i,t)$ if $\ui$ is unmatched at time $t$ with probability:
            \[
            \frac{1}{2 (1 - \nicefrac{1}{2} \cdot \sum_{t_i < s < t} \xit[s])}~.
            \]
        \end{itemize}
    }
    \item \textbf{Update the stages of offline vertices:} \\
    For every $i$ in stage $1$ (i.e., $t_i = \infty$), set $t_i = t$ and claim $i$ is moved to stage $2$ iff 
    \begin{equation}
    \label{eqn:switch_stage}
    \sum_{s \le t} \wit \cdot \tildxl_{is} \ge (1-\epsalg) \cdot \sum_{s} \wit \cdot \tildxl_{is}~,	
    \end{equation}
    where $\epsalg$ is a parameter to be optimized.
    \item \textbf{Update the weights for stage $2$ vertices:} \\
    For each $t_i = t$:
    \begin{enumerate}
        \item Sort edges $\{(j, s)\}$ that satisfy $(i, s) \notin L$, $x_{js} > 0$, and $s > t$ in descending order based on the value of $\widehat{w}_{is} - \widehat{w}_{js}$, where $\widehat{w}_{js} = 2 \cdot w_{js}$ for $(j,s) \in L$ and $\widehat{w}_{js} = w_{js}$ for $(j,s) \notin L$.
        \item For each edge $(j, s)$ in the above sorted list, let $\Delta_{i,j,s} = \min\{1 - \sum_{s'} x_{is'}, x_{js}\}$. Update $x_{is} \gets \Delta_{i,j,s}$ and $x_{js} \gets x_{js} - \Delta_{i,j,s}$.
        \item Stop the above loop when  $\sum_{s'} x_{is'}$ reaches $1$.
    \end{enumerate}
    %while $\sum_{s} \xit[s] < 1$ and $\max_{(i,s) \notin L, x_{js} > 0, s>t} \left( \widehat{w}_{is} - \widehat{w}_{js}\right) > 0$, let
    %\[
    %(j,s) = \argmax_{(i,s) \notin L, x_{js} > 0, s>t} \left( \widehat{w}_{is} - \widehat{w}_{js} \right)~,
    %\]
    %where $\widehat{w}_{it} = 2 \cdot \wit$ for $(i,t) \in L$ and $\widehat{w}_{it} = \wit$ for $(i,t) \notin L$.
    %Then, we reallocate an infinitesimal fraction of $dx$ from $(j,s)$ to $(i,s)$ by
    %\[
    %x_{is} \mathrel{{+}{=}} \dd x, \quad \text{and} \quad x_{js} \mathrel{{-}{=}} \dd x
    %\]
\end{enumerate}
\end{tcolorbox}


\subsection{Analysis of the Algorithm}

To begin, we introduce some important notations that shall be useful for our analysis.
\begin{itemize}
    \item For every $(i,s) \in E$ and $t \in V$, we use $x^{(t)}_{is}$ to denote the value of $x_{is}$ when $t$ arrives. We use $x^{\mathsf{last}}_{is}$ to denote the value when the instance ends. Note the following properties for $x^{(t)}_{is}$:
    \begin{itemize}
        \item For $(i, s) \in L$, $x^{(t)}_{is}$ is non-increasing with respect to $t$.
        \item The update of value $x^{(t)}_{is}$ stops when $t = s$, i.e., $x^{(t)}_{is} = x^{(s)}_{is}$ for $t \geq s$.
    \end{itemize}
    \item We define $E_1 = \{(i,t) : t \le t_i \}$ and $E_2 = \{(i,t) : t > t_i \}$ as a partition of the set of edges, i.e., $(i, t) \in E_1$ implies that vertex $i$ is still in stage $1$; $(i, t) \in E_2$ implies that $i$ moves to stage $2$.
    %We abuse $\xit$ to denote the value when the instance ends. 
    %\item For every $(i,t) \in L$, $x^{(s)}_{it}$ is non-increasing throughout the instance.
    %\item For every $(i,t) \in E$, $x^{(s)}_{it}$ is fixed after time $s \ge t$.
    %\item Let $E_1 = \{(i,t) : t \le t_i \}$ and $E_2 = \{(i,t) : t > t_i \}$.
%    \item Let $S_1, E_2 \setminus L / L_1, L_2$ be the sets of small/large edges that appear in stage $1$ and 2 respectively. That is,
%    \begin{align*}
%    & S_1 \eqdef \{ (i,t) \in S: t < t_i\}, \quad E_2 \setminus L \eqdef \{ (i,t) \in S: t > t_i \} \\
%    & L_1 \eqdef \{ (i,t) \in S: t < t_i\}, \quad L_2 \eqdef \{ (i,t) \in S: t \ge t_i \}~.
%    \end{align*}
%    Observe that the edge $(i,t_i)$ must be a large edge. For technical reason, we consider $(i,t)$ as a second stage large edge.
%    \item For every $U_0 \subseteq U$, let 
%    \begin{align*}
%    & S_1(U_0) \eqdef \{ (i,t) \in S: t < t_i, i \in U_0\}, \quad E_2 \setminus L(U_0) \eqdef \{ (i,t) \in S: t > t_i, i \in U_0 \} \\
%    & L_1(U_0) \eqdef \{ (i,t) \in S: t < t_i, i \in U_0\}, \quad L_2(U_0) \eqdef \{ (i,t) \in S: t \ge t_i, i \in U_0 \}~.
%    \end{align*}
\end{itemize}


Next, we provide the step-by-step analysis of the algorithm.




\paragraph{Online rounding. (Step 1 and 2)}
Recall that in the warm up section (the deterministic and free vertices setting), there is no component of rounding as we abstract out the random realization of online vertices.
Our rounding algorithm is rather straightforward. Upon the arrival of an online vertex $t$, it proposes to at most one of its neighbors, with probability $\nicefrac{\xit}{p_t}$ each.
Then, each offline vertex accept proposals greedily in stage $1$, and runs an $\nicefrac{1}{2}$-selectable online contention resolution scheme (OCRS) in stage $2$. The following lemma characterizes the loss of our rounding algorithm.

\begin{Lemma}
\label{lem:rounding}
\[
\alg \ge (1-\probfr) \cdot \left( \sum_{(i,t) \in E_1} \wit \cdot x^{(t)}_{it} + \frac{1}{2} \cdot \sum_{(i,t) \in E_2} \wit \cdot x^{(t)}_{it} \right)
\]
\end{Lemma}




\begin{proof}
We consider the contribution of each offline vertex $i$ to our algorithm separately.
Let $r_i = \Pr{i \text{ is matched in stage } 1}$. We first show that $r_i \le \probfr$:
\begin{align*}
r_i = \Pr{i \text{ is matched in stage }1} ~=&~ \Pr{i \text{ is proposed by some }t \le t_i} \\
=&~ 1 - \prod_{t \le t_i} (1-x^{(t)}_{it}) \le \sum_{t \le t_i} x^{(t)}_{it} \le \sum_{t \le t_i} \tildxl_{it} \le \probfr~,
\end{align*}
where we use the fact that $x^{(t)}_{it}$ is at most the initial value of $x_{it}$ when $(i,t) \in L$.
Then, the expected matching of $\ui$ from the first stage is
\begin{align*}
&\sum_{t\le t_i} \wit \cdot \Pr{\ui \text{ is proposed by } \vt } \cdot \Pr{i \text{ is unmatched before }t} \\
\ge~& \sum_{t\le t_i} \wit \cdot \Pr{\ui \text{ is proposed by } \vt } \cdot \Pr{i \text{ is unmatched at }t_i} \\
\ge~& \sum_{t\le t_i} \wit \cdot x^{(t)}_{it} \cdot (1 - \probfr) = (1-\probfr) \cdot \sum_{t: (i,t) \in E_1} \wit \cdot x^{(t)}_{it}~.
\end{align*}
Next, we consider the expected reward from the second stage. We prove by induction that every edge $(i,t)$ from the second stage (i.e., $t>t_i$) is matched with probability $\frac{1-r_i}{2}$. 
Suppose the statement holds for every $t_i < s <t$. Consider the edge $(i,t)$. According to the design of our algorithm, $(i,t)$ is selected with probability:
\begin{multline*}
\frac{1}{2 (1 - \frac{1}{2} \cdot \sum_{t_i < s < t} x^{(s)}_{is})} \cdot \Pr{\ui \text{ is proposed by } \vt } \cdot \Pr{i \text{ is unmatched before }t} \\
= \frac{1}{2 (1 - \frac{1}{2} \cdot \sum_{t_i < s < t} x^{(s)}_{is})} \cdot x^{(t)}_{it} \cdot \left(1 - r_i - \frac{1-r_i}{2} \cdot \sum_{t_i < s < t} x^{(s)}_{is} \right) = \frac{1-r_i}{2} \cdot x^{(t)}_{it}~,
\end{multline*}
where the first equation holds by induction hypothesis.
Therefore, the contribution from the second stage equals
\[
\sum_{t>t_i} \wit \cdot \frac{1-r_i}{2} \cdot \xit \ge (1-\probfr) \cdot \frac{1}{2} \cdot \sum_{t:(i,t) \in E_2} \wit \cdot \xit~.
\]
Summing the above equations over all $i \in U$ concludes the proof of the lemma.
\end{proof}

\paragraph{Fractional algorithm. (Step 3 and 4)} 
%The above bound is similar to equation~\eqref{??} of Section~\ref{sec:warmup}, despite that we loss a factor of $(1-\probfr)$ as the large edges now can have $\probfr$ mass instead of being ``free''; and an extra $\nicefrac{1}{2}$ factor for small edges as they are not necessarily ``deterministic''.
We are left to analyze our fractional algorithm. We shall prove that our fractional algorithm achieves a total reward of at least $0.625 - o(1)$. 

% Our fractional algorithm is non-adaptive to the realizations of the vertices. We initiate the solution with $\xit=\xit^*$ for large edges and $\xit=0$ for small edges.
% Every offline vertex starts with stage $1$, and keeps collecting large edges, until $(1-\epsalg)$ fraction of its corresponding large contributions (i.e., $\sum_{(i,t)\in L} \wit \cdot \xit^*$) is collected.
% At the moment when an offline vertex enters stage $2$, we run a ``online weighted matching with free disposal algorithm'' for collecting small edges.

Our analysis proceeds similarly as in Section~\ref{sec:warmup}. 
For each offline vertex, we keep collecting free edges until $1-\epsalg$ fraction of the free edges have arrived (refer to equation~\eqref{eqn:switch_stage}). According to the slackness check of our algorithm, intuitively, the optimal online algorithm should have the same behavior as solution $\tildx$, i.e., the optimal algorithm also only collect free edges in stage $1$, implying that each offline vertex is still free with high probability when switching to stage $2$, and the free edges are rarely picked in stage $2$.  As a result, the optimal algorithm collects a sufficiently high reward stage $2$ even if we exclude those large-value edges in $L$. Formally, we give the following \Cref{lem:opt_second}:
\begin{Lemma}
\label{lem:opt_second}
    $\sum_{(i,t) \in E_2 \setminus L} \wit \cdot \yit^* \ge  0.5 - \epsphilo - \epsu - \epsslack -4 \sqrt{\frac{\epsslack}{\epsalg}}$.
\end{Lemma}
\begin{proof}
Let $U_0 \subseteq U$ be the set of vertices that the optimal algorithm matches with probability less than $\delta$, i.e.,
\[
U_0 \eqdef \left\{ \ui \in U: \sum_{t < t_i} \yit^* \le \delta \right\} \quad \text{and} \quad \overline{U_0} \eqdef U \setminus U_0~,
\]
where $\delta$ is defined to be $\sqrt{\epsslack/\epsalg}$.
Since the realization of online vertex $t$ is independent to the event that an vertex $i$ is matched before $t$, we have that
\[
\yit^* \le p_t \cdot \left( 1 - \sum_{s<t} \yit[s]^* \right), \quad \forall \ui \in U, \vt \in V~.
\]
We remark that this is the crucial constraint of previous works~\cite{} for approximating the online optimum with known arrival orders.
Applying this inequality to $t \ge t_i$, we have that
\[
\frac{\yit^*}{p_t} \le 1 - \sum_{s<t} \yit[s]^* \le 1 - \sum_{s< t_i} \yit[s]^* \le 1-\delta , \quad \forall i \in \overline{U_0}, t \ge t_i~.
\]
Furthermore, since $\{\yit^*\}$ is a feasible solution of $\lpcore$, we have that
\begin{align*}
\epsslack \ge \lpcore & \ge \sum_{i,t} \wit \cdot \tildxl_{it} \cdot \left(1 - \frac{\yit^*}{p_t} \right) + \sum_{L} \wit \cdot \yit^* \cdot \left(1 - \frac{\tildxl_{it}}{p_t} \right) \\
& \ge \sum_{i \in \overline{U_0}} \sum_{t \ge t_i} \wit \cdot \tildxl_{it} \cdot \left(1 - \frac{\yit^*}{p_t} \right) + \sum_{L} \wit \cdot \yit^* \cdot \left(1 - \frac{\tildxl_{it}}{p_t} \right) \\
& \ge \delta \cdot \epsalg \cdot \sum_{i \in \overline{U_0}} \lp_i(\tildxl) + \sum_{L} \wit \cdot (\yit^* - \tildxl_{it})^+,
% & \ge \epsalg \cdot (\delta - \probfr) \cdot \left(0.5 - \epsl \right) \cdot \lp(\overline{U_0})
\end{align*}
where the last inequality uses the fact that online vertices $t \geq t_i$ contributes at least $\epsalg$ fraction of $\lp_i(\tildxl)$. Therefore, the above inequality gives
\begin{align*}
    \sum_{i \in \overline{U_0}} \lp_i(\tildxl) ~\leq~ \frac{\epsslack}{\delta \cdot \epsalg} \qquad \text{and} \qquad \sum_{L} \wit \cdot (\yit^* - \tildxl_{it})^+ ~\leq~ \epsslack.
\end{align*}


Now, we are ready to lower-bound $\sum_{(i,t)\in E_2 \setminus L} \wit \cdot \yit^*$. We have
\begin{align}
\label{eqn:philo_second}
\sum_{(i,t)\in E_2 \setminus L} \wit \cdot \yit^* &= \philo - \sum_{(i,t)\in E_1 \cup L} \wit \cdot \yit^* \notag \\
&\ge \philo - \sum_{(i,t) \in L} \wit \cdot \yit^* - \sum_{ (i,t) \in E_1 \setminus L \land i \in U_0} \wit \cdot \yit^* - \sum_{(i,t) \in E_1 \setminus L \land i \in \overline{U_0}} \wit \cdot \yit^* 
\end{align}

It remains to bound the three summations in \eqref{eqn:philo_second} separately. For the first summation, we have
\begin{align}
    \sum_{L} \wit \cdot \yit^* ~\leq~ \sum_{L} \wit \cdot \tildxl_{it} + \sum_{L} \wit \cdot (\yit^* - \tildxl_{it})^+ ~\leq~ \lp(\tildxl) + \epsslack. \label{eq:firstsum}
\end{align}
For the second summation, we have
\begin{align}
    \sum_{ (i,t) \in E_1 \setminus L \land i \in U_0} \wit \cdot \yit^* ~\leq~ \sum_{i \in U_0} \sum_{t: (i, t) \in E_1 \setminus L} 2\lp_i(\tildx) \cdot y^*_{it} ~\leq~ 2\delta \cdot \lp(\tildx), \label{eq:secondsum}
\end{align}
where the first inequality uses the fact that $w_{it} \leq 2\lp_i(x)$ for $(i,t) \notin L$, and the second inequality uses the fact that for every $i \in U_0$, we have
\[
\sum_{t:(i,t) \in E_1 \setminus L} y^*_{it} ~\leq~ \sum_{t < t_i} y^*_{it} ~\leq~ \delta.
\]
Here, we use a critical observation that $(i, t_i) \in L$.

For the third summation in \eqref{eqn:philo_second}, we have
\begin{align}
    \sum_{(i,t) \in E_1 \setminus L \land i \in \overline{U_0}} \wit \cdot \yit^*  ~\leq~ \sum_{i \in \overline{U_0}} \sum_{t: (i, t) \in E_1 \setminus L} 2\lp_i(\tildx) \cdot y^*_{it} ~\leq~ 2\sum_{i \in \overline{U_0}} \lp_i(\tildx) ~\leq~ \frac{2\epsslack}{\delta \cdot \epsalg}, \label{eq:thirdsum}
\end{align}
where the inequality uses the fact that $w_{it} \leq 2\lp_i(x)$ for $(i,t) \notin L$. 

Finally, applying the above \eqref{eq:firstsum}, \eqref{eq:secondsum} and \eqref{eq:thirdsum} to \Cref{eqn:philo_second} together with the assumption that $\philo \geq 1 - \epsphilo$ gives
\[
\sum_{(i,t)\in E_2 \setminus L} \wit \cdot \yit^* ~\geq~ 1 - \epsphilo - \lp(\tildxl) - \epsslack - 2\delta - \frac{2\epsslack}{\delta \cdot \epsalg} ~\geq~ 0.5 - \epsphilo - \epsu - \epsslack - 4\sqrt{\frac{\epsslack}{\epsalg}},
\]
where the last inequality uses the fact that $\lp(\tildxl) \leq (0.5 + \epsu) \cdot \lp(\tildx) \leq 0.5 + \epsu$ and that $\delta := \sqrt{\epsslack/\epsalg}$.
\end{proof}




Finally, we interpret the Step $4$ of our algorithm as an ``online weighted matching with free disposal'' algorithm for solving the below online problem.
\begin{itemize}
\item Only the set of large edges $L$ is given at the beginning, each with weight $\widehat{\wit} = 2 \wit$. Each vertex $\ui \in U$ has capacity $1$ and each vertex $\vt \in V$ has capacity $p_t$.
\item An initial matching is given as $x = \tildxl$.
\item At time $t_i$ (in ascending order of $t_i$), the edge set $E_2 \setminus L(i) = \{(i,t) \in S: t > t_i \}$ is observed, each with weight $\widehat{\wit} = \wit$. The algorithm (fractionally) matches edges in $E_2 \setminus L(i)$ immediately. Previously selected edges (including those larges edges provided at the beginning) can be freely disposed of, while they cannot be retrieved once we proceeds to the next time step.
\item The goal is to maximize the total increment over the original matching.
\end{itemize}
The offline optimum of the above problem can be characterized as the following linear program.
\begin{align*}
\max: \quad & \sum_{(i,t) \in E} \widehat{\wit} \cdot (\tildz_{it} - \tildxl_{it}) & \lpsecond \\
% + \sum_{(i,t) \in E_1} \widehat{\wit} \cdot (\tildz_{it} - \tildxl_{it}) & \lpsecond \\
\text{subject to}: \quad & \sum_{t:(i,t) \in E_2 \setminus L} \tildz_{it} + \sum_{t:(i,t) \in L} \tildz_{it} \le 1 & \forall \ui \in U \\
& \sum_{i:(i,t) \in E_2 \setminus L} \tildz_{it} + \sum_{i:(i,t) \in L} \tildz_{it} \le p_t & \forall \vt \in V \\
& \tildz_{it} \le \tildxl_{it} & \forall (i,t) \in L
\end{align*}
\enze{the last line was $\tildz_{it} \le \xit^*  \forall (i,t) \in L$}

We establish in the following lemma that our algorithm (Step 4) achieves at least half of $\lpsecond$. We remark that our algorithm is essentially a greedy algorithm that always continuously matches the edge with the largest marginal increment. The ratio $\nicefrac{1}{2}$ follows from a standard analysis and can be improved to $1-\nicefrac{1}{e}$ via a more careful fractional algorithm (refer to \cite{???}). 
\begin{Lemma}
\label{lem:alg_free_disposal}
\[
\sum_{(i,t) \in E_2 \setminus L} \wit \cdot \xit  + \sum_{(i,t) \in L} 2 \cdot \wit \cdot (\xit - \tildxl_{it}) \ge \frac{1}{2} \cdot \lpsecond
\]
\end{Lemma}
\begin{proof}
\zhihao{move the proof to appendix. Please complete the proof.}
We use $\Delta\alg(t_i)$ to denote the marginal gain of our algorithm at time $t_i$.
\begin{align*}
\Delta\alg(t_i) & = \sum_{t:(i,t) \in E_2 \setminus L} \int_0^{\xit(t_i)} (\wit - w_t(t_i, s)) \dd s \ge \sum_{(i,t) \in E_2 \setminus L} \int_0^{\tildz_{it}^*} (\wit - w_t(t_i, s)) \dd s \\
& = \sum_{(i,t) \in E_2 \setminus L} \int_0^{\tildz_{it}^*} (\wit - w_t(0, s)) \dd s + \sum_{(i,t) \in E_2 \setminus L} \int_0^{\tildz_{it}^*} (w_t(0,s) - w_t(t_i, s)) \dd s
\end{align*}
\end{proof}
\enze{
comments: $\int_0^{\tildz_{it}^*} w_t(0,s) - w_t(t_i, s) $ is hard to bound because $w_t(t_i, s)$ is about $\xit(t_i)$ but $\int_0^{\tildz_{it}^*}$.
}
\begin{proof}
We can arbitrarily split every online vertex $t$ into $|V|+1$ vertices, named $v_{it}(i \in \{0,1,2,...,|V|\})$. the capacity $v_{it}$ is $\tildz_{it}^*$ while $i \neq 0$, and $p_t- \sum_i \tildz_{it}^*$ while $i = 0$


We use $\Delta\alg(t_i)$ to denote the marginal gain of our algorithm at time $t_i$. Then we have
$$\Delta\alg(t_i) \geq \sum_{(i,s) \in E_2 \setminus L} \sum_j x(j,v_{it},t_i) (\wit - w_{jt})$$
where $x(j,v_{it},t_i)$ means the $x_{j,v_{it}}$ in the algorithm at time $t_i$. Because in the algorithm the $x(j,v_{it},t_i)$ is monotonically increasing,
$$x(j,v_{it},t_i) \leq x(j,v_{it},1)$$

Therefore,
\begin{align*}
    &\sum_{(i,t) \in E_2 \setminus L} \wit \cdot \xit  + \sum_{(i,t) \in L} 2 \cdot \wit \cdot (\xit - \tildxl_{it})\\
    =& \sum_{i}\Delta\alg(t_i) \geq \sum_{(i,t) \in E_2 \setminus L} \sum_j x(j,v_{it},t_i) (\wit - w_{jt})\\
    = &\sum_{(i,t) \in E_2 \setminus L} \sum_j x(j,v_{it},t_i) \wit - \sum_{(i,t) \in E_2 \setminus L} \sum_j x(j,v_{it},t_i) w_{jt}\\
    \geq &\sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^* \wit - \sum_{(i,t) \in E_2 \setminus L} \sum_j x(j,v_{it},1) w_{jt}\\
    =&\sum_{(i,t) \in E_2 \setminus L} \Big(\tildz_{it}^* \wit-\sum_j x(j,v_{it},0) w_{jt} \Big) - \sum_{(i,t) \in E_2 \setminus L} \Big(\sum_j x(j,v_{it},0) w_{jt}-\sum_j x(j,v_{it},1) w_{jt} \Big) 
\end{align*}

We have
$$\sum_{(i,t) \in E_2 \setminus L} \Big(\tildz_{it}^* \wit-\sum_j x(j,v_{it},0) w_{jt} \Big) = \lpsecond$$
and
\begin{align*}
&\sum_{(i,t) \in E_2 \setminus L} \Big(\sum_j x(j,v_{it},0) w_{jt}-\sum_j x(j,v_{it},1) w_{jt} \Big)  \\
\leq& \sum_{(i,t)} \Big(\sum_j x(j,v_{it},0) w_{jt}-\sum_j x(j,v_{it},1) w_{jt} \Big)\\
= &\sum_{i}\Delta\alg(t_i)  = \sum_{(i,t) \in E_2 \setminus L} \wit \cdot \xit  + \sum_{(i,t) \in L} 2 \cdot \wit \cdot (\xit - \tildxl_{it})
\end{align*}
\end{proof}
% Notation:
% \begin{itemize}
%     \item $\hat{w}_t(t_i, r)$ $r$-least of $\forall j, \hat{w}_{jt}$ at time $t_i$
%     \item $\Delta_x \in \tildz_{it}^*$ the infinitesimal fraction $\Delta_x$ finally allocated to $\tildz_{it}^*$ in $\opt$.
%     \item $\hat{w}_{\Delta_x}(t_i)$ the weight of vertex $i$ which the infinitesimal fraction $\Delta_x$ allocates to at time $t_i$
% \end{itemize}
% \begin{proof}
% We use $\Delta\alg(t_i)$ to denote the marginal gain of our algorithm at time $t_i$.
% % \begin{align*}
% % \sum_i \Delta\alg(t_i) =&  \sum_{(i,t) \in E_2 \setminus L} \int_0^{\xit(t_i)} (\wit - w_t(t_i, s)) \dd s \ge \sum_{(i,t) \in E_2 \setminus L} \int_0^{\tildz_{it}^*} (\wit - w_t(t_i, s)) \dd s \\
% % =&\sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^*\wit - \sum_{(i,t) \in E_2 \setminus L} \int_0^{\tildz_{it}^*}  w_t(t_i, s) \dd s \\
% % \geq&\sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^*\wit - \sum_{(i,t) \in E_2 \setminus L} \frac{\tildz_{it}^*}{p_t} \int_0^{p_t}  w_t(t_i, s) \dd s \\
% % \geq& \sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^*\wit - \alg \\
% % \end{align*}
% % $$\alg = \sum_t \int_0^{p_t} w_t(t,s) \dd s $$
% \begin{align*}
% \sum_i \Delta\alg(t_i) =&  \sum_{(i,t) \in E_2 \setminus L} \int_0^{\xit(t_i)} (\wit - \hat{w}_t(t_i, r)) \dd r \ge \sum_{(i,t) \in E_2 \setminus L} \int_0^{\tildz_{it}^*} (\wit - \hat{w}_t(t_i, r)) \dd r \\
% \geq&\sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^*\wit - \sum_{(i,t) \in E_2 \setminus L} \int_{\tildz_{it}^*} \hat{w}_{\Delta_x}(t_i) \dd r\\
% \geq&\sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^*\wit - \sum_{(i,t) \in E_2 \setminus L} \int_{\tildz_{it}^*} \hat{w}_{\Delta_x}(1) \dd \Delta_x\\
% = &\left(\sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^*\wit  - \sum_{(i,t) \in E_2 \setminus L} \int_{\tildz_{it}^*} \hat{w}_{\Delta_x}(0) \dd \Delta_x \right)- \sum_{(i,t) \in E_2 \setminus L} \int_{\tildz_{it}^*} (\hat{w}_{\Delta_x}(1)-\hat{w}_{\Delta_x}(0)) \dd \Delta_x\\
% \end{align*}
% Because we have
% $$\sum_{(i,t) \in E_2 \setminus L} \int_{\tildz_{it}^*} (\hat{w}_{\Delta_x}(1)-\hat{w}_{\Delta_x}(0)) \dd \Delta_x \leq \sum_{(i,t)} \int_{\tildz_{it}^*} (\hat{w}_{\Delta_x}(1)-\hat{w}_{\Delta_x}(0)) \dd \Delta_x = \sum_i \Delta\alg(t_i) $$
% Also,
% $$\sum_{(i,t) \in E_2 \setminus L} \tildz_{it}^*\wit  - \sum_{(i,t) \in E_2 \setminus L} \int_{\tildz_{it}^*} \hat{w}_{\Delta_x}(0) \dd \Delta_x = \lpsecond$$
% Therefore,
% $$\sum_{(i,t) \in E_2 \setminus L} \wit \cdot \xit  + \sum_{(i,t) \in L} 2 \cdot \wit \cdot (\xit - \xit^*) \geq \lpsecond - \left(\sum_{(i,t) \in E_2 \setminus L} \wit \cdot \xit  + \sum_{(i,t) \in L} 2 \cdot \wit \cdot (\xit - \xit^*)\right)$$
% \end{proof}
\subsection{Proof of Theorem~\ref{thm:lp_uniq_small}}
We are now ready to complete the proof of Theorem~\ref{thm:lp_uniq_small}.

\begin{proof}[Proof of \Cref{thm:lp_uniq_small}]
Recall that \Cref{lem:rounding} gives
    \begin{align}
\label{eqn:alg_uniq_small}
\alg & \ge  (1-\probfr) \cdot \left( \sum_{(i,t) \in E_1} \wit \cdot x^{(t)}_{it} + \frac{1}{2} \cdot \sum_{(i,t) \in E_2} \wit \cdot x^{(t)}_{it} \right) \notag \\
& \ge (1-\probfr) \cdot \left( \sum_{(i,t) \in E_1} \wit \cdot \tildxl_{it} + \frac{1}{2} \cdot \sum_{(i,t) \in E_2 \setminus L} \wit \cdot x^{(t)}_{it} + \sum_{(i,t) \in L} \wit \cdot (x^{(t)}_{it} -\tildxl_{it}) \right) \notag \\
& \ge (1-\probfr) \cdot \left( (1-\epsalg) \cdot \lp(\tildxl) + \frac{1}{4} \cdot \lpsecond \right)~, 
\end{align}
where the first inequality holds by Lemma~\ref{lem:rounding}, the second inequality uses the fact that in stage $1$ we only collect rewards from $(i, t) \in E_1 \cap L$ and the fact that $x^{(t)}_{it} \leq \tildxl_{it}$ for $(i,t) \in E_2 \cap L$, and the last inequality holds by the the design of our algorithm and \Cref{lem:alg_free_disposal}.

It remains to lower-bound the value of $\lpsecond$. Note that the following feasible solution of program $\lpsecond$:
\[
\tildz_{it} = \begin{cases} \min(\tildxl_{it}, \yit^*) & (i,t) \in E_1  \\\yit^* & (i,t) \in E_2 \setminus L \\ 0 & (i,t) \in E_2 \cap L
\end{cases}~.
\]
Therefore, we have
\begin{align*}
\lpsecond & \ge \sum_{(i,t) \in E_2} \widehat{\wit} \cdot \tildz_{it} + \sum_{(i,t) \in E_1} \widehat{\wit} \cdot (\tildz_{it} - \tildxl_{it}) \\
& \ge \sum_{(i,t) \in E_2} \wit \cdot \yit^* - \sum_{(i,t) \in L} 2 \cdot \wit \cdot (\tildxl_{it} - \yit^*)^+ \\
&\ge 0.5 - \epsphilo - \epsu - \epsslack -4 \sqrt{\frac{\epsslack}{\epsalg}} - 2\epsslack,
\end{align*}
where the last inequality holds by Lemma~\ref{lem:opt_second} and the observation that
\[
\epsslack ~\geq~ \sum_{(i,t) \in L} w_{it} \tildxl_{it} \cdot (1 - y^*_{it}/p_t) ~\geq~ \sum_{(i,t) \in L} w_{it} \cdot (\tildxl_{it} - y^*_{it})^+.
\]
. Applying the bound on $\lpsecond$ to \eqref{eqn:alg_uniq_small}, we have 
\begin{align*}
    \alg ~&\geq~ (1-\probfr) \cdot \left( (1-\epsalg) \cdot \lp(\tildxl) + \frac{1}{4} \cdot \left( 0.5 - \epsphilo - \epsu - 3\epsslack -4 \sqrt{\frac{\epsslack}{\epsalg}} \right) \right) \\
    ~&\geq~ 0.625 - \probfr - \frac{\epsalg}{2} - \epsl - \frac{\epsphilo + \epsu + 3\epsslack}{4} - \sqrt{\frac{\epsslack}{\epsalg}}  \\
    ~&\geq~ 0.625 - 1.5 \epsslack^{1/3} - \epsphilo - \epsu - 3\epsslack,
\end{align*}
where the last inequality is satisfied when taking $\epsalg = \epsslack^{1/3}$.
\end{proof}


% \begin{align*}
% \max: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \cdot \wit + \sum_{(i,t)\in E_2 \setminus L, (j,t) \in L} z_{i,jt} \cdot \left( \wit - \alpha \cdot w_{jt} \right) \\
% \text{subject to}: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} + \sum_{(i,t) \in E_2 \setminus L , (j,t) \in L} z_{i,jt} \le 1 & \forall u_i \in U \\
% & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \le p_t - x_{L,t}^* & \forall v_t \in V \\
% & \sum_{i:(i,t) \in E_2 \setminus L} z_{i,jt} \le (x_{jt}^* -  y_{jt}^*)^+& \forall (j,t) \in L \\
% \end{align*}


% Notice that 
% \[
% \sum_{(i,t)\in E_2 \setminus L, (j,t) \in L} z_{i,jt}  \cdot w_{jt} \le \sum_{(j,t)\in L}(x_{jt}^* -  y_{jt}^*)^+ \cdot w_{jt} \le  \zhihao{o(1), todo}
% \]

% \begin{align*}
% \max: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \cdot \wit + \sum_{(i,t)\in E_2 \setminus L, (j,t) \in L} z_{i,jt} \cdot \wit \\
% \text{subject to}: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} + \sum_{(i,t) \in E_2 \setminus L , (j,t) \in L} z_{i,jt} \le 1 & \forall u_i \in U \\
% & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \le p_t - x_{L,t}^* & \forall v_t \in V \\
% & \sum_{i:(i,t) \in E_2 \setminus L} z_{i,jt} \le (x_{jt}^* -  y_{jt}^*)^+& \forall (j,t) \in L \\
% \end{align*}

% \begin{align*}
% \max: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \cdot \wit\\
% \text{subject to}: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \le 1 & \forall u_i \in U \\
% & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \le p_t - x_{L,t}^* + \sum_{j:(j,t) \in L} (x_{jt}^* -  y_{jt}^*)^+ & \forall v_t \in V \\
% \end{align*}

% \begin{align*}
% \max: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \cdot \wit\\
% \text{subject to}: \quad & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it}  \le 1 & \forall u_i \in U \\
% & \sum_{(i,t) \in E_2 \setminus L} \tildz_{it} \le p_t - y_{L,t}^* & \forall v_t \in V \\
% \end{align*}

% We suppose $t_i$ means the time of offline vertex $i 
% \in U$ achieve $1-\ezeps$ of $\sum_{t:(i,t) \in L} x_{it}^*$, formally,
% $$\sum_{t: t \leq t_i, (i,t) \in L} x_{it}^* \geq\sum_{t:(i,t) \in L} x_{it}^*\quad \text{and}\quad \sum_{t: t < t_i, (i,t) \in L} x_{it}^* <\sum_{t:(i,t) \in L} x_{it}^*$$

% Because $t_i$ only depends on the information at and before $t_i$, whether $t = t_i$ can be check online.

% Next, we will consider a classic algorithm that online weighted matching with free disposal. The model is as follows:

% Online vertices are $U \cup L$. 

% \begin{algorithm}
% \caption{}
% Initialization:\\
% $x_{it} = \begin{cases}
%     x^*_{it} & ((it) \in L)\\
%     0 & ((it) \in S)\\
% \end{cases}$\\
% $x_{0t} = p_t - x^*_{Lt}$
% \\
% $t_i \gets \infty$
% \\
% \For{arrival of $\vt$} {
%   propose to $\ui$ w.p. $\frac{x_{it}}{p_t}$\\
%   \For{$\ui \in U$}{
%     \If{receives a proposal from $\vt$}{
%         \eIf{$t \leq t_i$}{
%             ...%greedy
%         }{
%             ...%1/2-OCRS
%         }
%     }
%   }
%   \For{$i:(1-\ezeps)\sum_{t:(i,t) \in L} w_{it} x_{it}^* \in \left(\sum_{t': t' < t, (i,t') \in L} w_{it} x_{it}^* ,\sum_{t: t \leq t_i, (i,t) \in L} w_{it} x_{it}^* \right]$}{
%     $t_i \gets t$\\
%     $s \gets 1-\delta$\\
%     \While{$s>0$}{
%        $(i^*,t^*) \gets \arg\max_{t^*>t, x_{i^*t^*}>0}w_{it^*} - \widetilde{w_{i^*t^*}}$\\
%        \Bigg(where $\widetilde{w_{i^*t^*}} = \begin{cases}
%        0  &i^* = 0\\
%        w_{i^*t^*}  &(i^*t^*) \in S\\
%        \alpha w_{i^*t^*}  &(i^*t^*) \in L\\
%        \end{cases}$\Bigg)\\
%        \If{$w_{it^*} - \widetilde{w_{i^*t^*}}<0$}{
%           break;
%        }
%        $dx_{ii^*t^*} \gets \min \{s, x_{i^*t^*}\}$\\
%        $s \gets s - dx_{ii^*t^*}$\\
%        $x_{i^*t^*} \gets x_{i^*t^*} - dx_{ii^*t^*}$\\
%        $x_{it^*} \gets x_{it^*} + dx_{ii^*t^*}$\\
%     }
%   }
% }
% \end{algorithm}

% \begin{Lemma}
%     $\alg_\delta = \sum_{(it) \in E_2 \setminus L} x_{it} w_{it} - \alpha \sum_{(it) \in E_2 \setminus L} (x^*_{it} - x_{it}) w_{it}  \geq \frac12 LP_\text{2nd-stage}$
% \end{Lemma}
% \begin{proof}
% We suppose the solution of LP is $z$.
% Therefore, $\opt = \sum_{(it) \in E_2 \setminus L} z_{it} w_{it} - \alpha \sum_{(it) \in L} (x*_{it} - z_{it}) w_{it}$
% % \begin{align*}
% %     &\alg\\
% %     =&\sum_{(it) \in E_2 \setminus L} x_{it} w_{it} - \alpha \sum_{(it) \in L} (x*_{it} - x_{it}) w_{it} \\
% %     =& \sum_t \sum_{i:t_i = t} \sum_{i^*t^*}dx_{iti^*t^*} (w_{it^*} - \widetilde{w_{i^*t^*}})\\
% %     \geq& \sum_t \sum_{i:t_i = t} \max_{i^*: x^{(t+1)}_{i^*t(i)}>0} (w_{it(i)} - \widetilde{w_{i^*t(i)}})\\
% %     \geq& \sum_t \sum_{i:t_i = t} \max_{i^*: x^\text{End}_{i^*t(i)}>0} (w_{it(i)} - \widetilde{w_{i^*t(i)}})\\
% %     =& \sum_t \sum_{i:t_i = t} w_{it(i)} - \sum_t \sum_{i:t_i = t} \min_{i^*: x^\text{End}_{i^*t(i)}>0} \widetilde{w_{i^*t(i)}}\\
% %     \geq& \opt - \alg
% % \end{align*}
% According to the process of the algorithm,
% \begin{align*}
%     &\alg_\delta\\
%     =&\sum_{(it) \in E_2 \setminus L} x_{it} w_{it} - \alpha \sum_{(it) \in L} (x^*_{it} - x_{it}) w_{it} \\
%     =& \sum_i \sum_{i^*t^*}dx_{ii^*t^*} (w_{it^*} - \widetilde{w_{i^*t^*}})\\
% \end{align*}
% Also, in the algorithm we always choose the $i^* t^*$ with maximum $w_{it^*} - \widetilde{w_{i^*t^*}}$ that $x^(t)_{i^* t^*} > 0$. When we consider $it$, there are two pairs $i^*t^*$, $i't'$ satisfy that $dx_{ii^*t^*} > 0,x^{(t+1)}_{i't'}>0$, due to the algorithm, we have
% $$w_{it^*} - \widetilde{w_{i^*t^*}} \geq w_{it'} - \widetilde{w_{i't'}}$$
% First, for any $i$, we consider $\sum_{i^*t^*} dx_{ii^*t^*}$ and $\sum_{t^*} z_{it^*}$. When $\max_{i^*t^*: x^{(t+1)}_{i^*t^*}>0} (w_{it^*} - \widetilde{w_{i^*t^*}}) > 0$, we have $\sum_{i^*t^*} dx_{ii^*t^*} = 1 - \delta \geq \sum_{t^*} z_{it^*}$. Therefore
% \begin{align*}
%     &\alg_\delta\\
%     =& \sum_i \sum_{i^*t^*}dx_{ii^*t^*} (w_{it^*} - \widetilde{w_{i^*t^*}})\\
%     \geq& \sum_i \sum_{t^*} z_{it^*}\max_{i^*: x^{(t+1)}_{i^*t^*}>0} (w_{it^*} - \widetilde{w_{i^*t^*}})\\
%     \geq& \sum_i \sum_{t^*} z_{it^*}\max_{i^*: x^\text{End}_{i^*t^*}>0} (w_{it^*} - \widetilde{w_{i^*t^*}})\\
%     =& \sum_i \sum_{t^*} z_{it^*} w_{it^*} - \sum_i \sum_{t^*} z_{it^*}\min_{i^*: x^\text{End}_{i^*t^*}>0} \widetilde{w_{i^*t^*}}\\
%     \geq& \sum_i \sum_{t^*} z_{it^*} w_{it^*} - \sum_{t^*} \min_{i^*: x^\text{End}_{i^*t^*}>0} \widetilde{w_{i^*t^*}}\\
%     \geq& LP_\text{2nd-stage} - \alg_\delta
% \end{align*}
% So we have
% $$\alg_\delta \geq \frac12 LP_\text{2nd-stage}$$
% \end{proof}

==> smallslack_bak2.tex <==
\section{Small slackness}
\label{sec:small_slackness}

In this section, we study the case when the slackness of instance is small and prove the following \Cref{thm:lp_uniq_small}:



\begin{Theorem}
\label{thm:lp_uniq_small}
    If $\philo \ge (1-\epsphilo) \cdot \lpexante$ and $\lpcore \le \epsslack$, there exists an order-unaware algorithm that collects an expected reward of $TBD$.
\end{Theorem}

\subsection{Our Algorithm}

Our algorithm consists of two components: 1) an online algorithm that maintains a fractional solution $\{\xit\}$ of the instance; 2) an online rounding algorithm applying to our fractional solution. 

The formal description of our algorithm is provided below. It is a generalization of the algorithm described in Section~\ref{sec:warmup}.
\begin{tcolorbox}[title=Algorithm when $\lpcore$ is small] 
Initialization:
\begin{enumerate}[(1)]
    \item Initiate $\xit = \tildxl_{it}$ for every $(i,t) \in E$. 
    \item Initiate $t_i = \infty$ for every $i \in U$. If $t \le t_i$, we say vertex $\ui$ is in the first stage, else we say $\ui$ is in the second stage. Initially, all offline vertices are in the first stage.
    \item For notation simplicity, we introduce a dummy offline vertex $0$ with $w_{0t} = 0$ for every $t \in V$, and let 
    \[
    x_{0t} = p_t - \sum_{i} \xit~.
    \]
    During the algorithm, condition $q_t(x) = p_t$ is always satisfied.
\end{enumerate}
\vspace{0.5cm}

Upon the arrival of $\vt$:
\begin{enumerate}[Step 1:]
    \item Let $\vt$ propose to $\ui$ with probability $\frac{\xit}{p_t}$ if $\vt$ is realized.
    \item If $\ui$ receives a proposal from $\vt$:
        %\begin{itemize}
         %   \item if $t \le t_i$, greedily select the edge $(i,t)$ if $\ui$ is unmatched at time $t$;
            %\item if $t > t_i$, select the edge $(i,t)$ if $\ui$ is unmatched at time $t$ with probability:
            %\[
            %\frac{1}{2 (1 - \nicefrac{1}{2} \cdot \sum_{t_i < s < t} \xit[s])}~.
            %\]
        %\end{itemize}
    \yifan{
        \begin{itemize}
            \item if $t_i = \infty$, greedily select the edge $(i,t)$ if $\ui$ is unmatched at time $t$;
            \item Otherwise, select the edge $(i,t)$ if $\ui$ is unmatched at time $t$ with probability:
            \[
            \frac{1}{2 (1 - \nicefrac{1}{2} \cdot \sum_{t_i < s < t} \xit[s])}~.
            \]
        \end{itemize}
    }
    \item \textbf{Update the stages of offline vertices:} \\
    For every $i$ in stage $1$ (i.e., $t_i = \infty$), set $t_i = t$ and claim $i$ is moved to stage $2$ iff 
    \begin{equation}
    \label{eqn:switch_stage}
    \sum_{s \le t} \wit \cdot \tildxl_{is} \ge (1-\epsalg) \cdot \sum_{s} \wit \cdot \tildxl_{is}~,	
    \end{equation}
    where $\epsalg$ is a parameter to be optimized, 
    \item \textbf{Update the weights for stage $2$ vertices:} \\
    For each $t_i = t$:
    \begin{enumerate}
        \item Sort edges $\{(j, s)\}$ that satisfy $(i, s) \notin L$, $x_{js} > 0$, and $s > t$ in descending order based on the value of $\widehat{w}_{is} - \widehat{w}_{js}$, where $\widehat{w}_{js} = 2 \cdot w_{js}$ for $(j,s) \in L$ and $\widehat{w}_{js} = w_{js}$ for $(j,s) \notin L$.
        \item For each edge $(j, s)$ in the above sorted list, let 
        \[
        \textstyle \Delta_{i,j,s} = \min\{1 - \probfr -  \sum_{s': (i, s') \notin L} x_{is'}, x_{js}\}~.
        \]. Update $x_{is} \gets \Delta_{i,j,s}$ and $x_{js} \gets x_{js} - \Delta_{i,j,s}$.
        \item Stop the above loop when  $\sum_{s': (i,s') \notin L} x_{is'}$ reaches $1 - \probfr$.
    \end{enumerate}
    %while $\sum_{s} \xit[s] < 1$ and $\max_{(i,s) \notin L, x_{js} > 0, s>t} \left( \widehat{w}_{is} - \widehat{w}_{js}\right) > 0$, let
    %\[
    %(j,s) = \argmax_{(i,s) \notin L, x_{js} > 0, s>t} \left( \widehat{w}_{is} - \widehat{w}_{js} \right)~,
    %\]
    %where $\widehat{w}_{it} = 2 \cdot \wit$ for $(i,t) \in L$ and $\widehat{w}_{it} = \wit$ for $(i,t) \notin L$.
    %Then, we reallocate an infinitesimal fraction of $dx$ from $(j,s)$ to $(i,s)$ by
    %\[
    %x_{is} \mathrel{{+}{=}} \dd x, \quad \text{and} \quad x_{js} \mathrel{{-}{=}} \dd x
    %\]
\end{enumerate}
\end{tcolorbox}


\subsection{Analysis of the Algorithm}

To begin, we introduce some important notations that shall be useful for our analysis.
\begin{itemize}
    \item For every $(i,s) \in E$ and $t \in V$, we use $x^{(t)}_{is}$ to denote the value of $x_{is}$ when $t$ arrives. 
    %We use $x^{\mathsf{last}}_{is}$ to denote the value when the instance ends. 
    Note the following properties for $x^{(t)}_{is}$:
    \begin{itemize}
        \item For $(i, s) \in L$, $x^{(t)}_{is}$ is non-increasing with respect to $t$, i.e., $x^{(t)}_{i,s} \leq \tildxl_{is}$ for every $t$. 
        \item For $(i, s) \notin L$, $x^{(t)}_{is} \leq x^{(t_i)}_{is}$. 
        \item The above two properties imply $\sum_{s \in V} x^{(t)}_{is} \leq \sum_{s: (i, s) \notin L} x^{(t_i)}_{is} + \probfr \leq 1$. Therefore, in Step 2 the matching probability is feasible since $ \frac{1}{2 (1 - \nicefrac{1}{2} \cdot \sum_{t_i < s < t} \xit[s])}$ is bounded by $1$.
    \end{itemize}
    \item We define $E_1 = \{(i,t) : t \le t_i \}$ and $E_2 = \{(i,t) : t > t_i \}$ as a partition of the set of edges, i.e., $(i, t) \in E_1$ implies that vertex $i$ is still in stage $1$; $(i, t) \in E_2$ implies that $i$ moves to stage $2$.
    %We abuse $\xit$ to denote the value when the instance ends. 
    %\item For every $(i,t) \in L$, $x^{(s)}_{it}$ is non-increasing throughout the instance.
    %\item For every $(i,t) \in E$, $x^{(s)}_{it}$ is fixed after time $s \ge t$.
    %\item Let $E_1 = \{(i,t) : t \le t_i \}$ and $E_2 = \{(i,t) : t > t_i \}$.
%    \item Let $S_1, E_2 \setminus L / L_1, L_2$ be the sets of small/large edges that appear in stage $1$ and 2 respectively. That is,
%    \begin{align*}
%    & S_1 \eqdef \{ (i,t) \in S: t < t_i\}, \quad E_2 \setminus L \eqdef \{ (i,t) \in S: t > t_i \} \\
%    & L_1 \eqdef \{ (i,t) \in S: t < t_i\}, \quad L_2 \eqdef \{ (i,t) \in S: t \ge t_i \}~.
%    \end{align*}
%    Observe that the edge $(i,t_i)$ must be a large edge. For technical reason, we consider $(i,t)$ as a second stage large edge.
%    \item For every $U_0 \subseteq U$, let 
%    \begin{align*}
%    & S_1(U_0) \eqdef \{ (i,t) \in S: t < t_i, i \in U_0\}, \quad E_2 \setminus L(U_0) \eqdef \{ (i,t) \in S: t > t_i, i \in U_0 \} \\
%    & L_1(U_0) \eqdef \{ (i,t) \in S: t < t_i, i \in U_0\}, \quad L_2(U_0) \eqdef \{ (i,t) \in S: t \ge t_i, i \in U_0 \}~.
%    \end{align*}
\end{itemize}


Next, we provide the step-by-step analysis of the algorithm.




\paragraph{Online rounding. (Step 1 and 2)}
Recall that in the warm up section (the deterministic and free vertices setting), there is no component of rounding as we abstract out the random realization of online vertices.
Our rounding algorithm is rather straightforward. Upon the arrival of an online vertex $t$, it proposes to at most one of its neighbors, with probability $\nicefrac{\xit}{p_t}$ each.
Then, each offline vertex accept proposals greedily in stage $1$, and runs an $\nicefrac{1}{2}$-selectable online contention resolution scheme (OCRS) in stage $2$. The following lemma characterizes the loss of our rounding algorithm.

\begin{Lemma}
\label{lem:rounding}
\[
\alg \ge (1-\probfr) \cdot \left( \sum_{(i,t) \in E_1} \wit \cdot x^{(t)}_{it} + \frac{1}{2} \cdot \sum_{(i,t) \in E_2} \wit \cdot x^{(t)}_{it} \right)
\]
\end{Lemma}

Intuitively, our algorithm collects almost entire  value of $w_{it} \cdot x^{(t)}_{it}$ when $i$ is in stage $1$, as $i$ is only matched to free edges. Therefore, the probability that $i$ got matched in stage $1$ should be bounded by $\probfr$. When $i$ moves to stage $2$, the OCRS framework guarantees that half of the value $w_{it} \cdot x^{(t)}_{it}$ is collected. We deferred the detailed proof of \Cref{lem:rounding} to TBD.




\yifan{Give some high-level intuition for $x$ before the algorithm.}
\paragraph{Fractional solution. (Step 3 and 4)} 


We are left to analyze our fractional solution $x$. We shall prove that our fractional algorithm achieves a total reward of at least $0.625 - o(1)$. 


Our analysis proceeds similarly as in Section~\ref{sec:warmup}. 
For each offline vertex, we keep collecting free edges until $1-\epsalg$ fraction of the free edges have arrived (refer to equation~\eqref{eqn:switch_stage}). According to the slackness check of our algorithm, intuitively, the optimal online algorithm should have the same behavior as solution $\tildx$, i.e., the optimal algorithm also only collect free edges in stage $1$, implying that each offline vertex is still free with high probability when switching to stage $2$, and the free edges are rarely picked in stage $2$.  As a result, the optimal algorithm collects a sufficiently high reward stage $2$ even if we exclude those large-value edges in $L$. Formally, we give the following \Cref{lem:opt_second}:
\begin{Lemma}
\label{lem:opt_second}
    $\sum_{(i,t) \in E_2 \setminus L} \wit \cdot \yit^* \ge  0.5 - \epsphilo - \epsu - \epsslack -4 \sqrt{\frac{\epsslack}{\epsalg}}$.
\end{Lemma}

We defer the proof of \Cref{lem:opt_second} to TBD.



\yifan{Only leave Lemma 6.5 as "x >= y*". The dirty notations will be placed in appendix. }

Finally, we interpret the Step $4$ of our algorithm as an ``online submodular welfare maximization'' process. To be specific, consider the following way to understand the Step $4$ of our algorithm: Define function $f_t$ as a function of $\{\tildz_{it}\}_{i:(i, t) \notin L}$, while parameterized by $\{\tildxl_{it}\}_{i:(i, t) \in L}$. To be specific, define
$\widehat w_{it}$ is defined as follows:
\[
\widehat w_{it} = \begin{cases} 2\cdot w_{it} & (i,t) \in L  \\ w_{it} & (i,t) \in E_2 \setminus L \\ 0 & (i,t) \in E_1 \setminus L
\end{cases}~.
\]
Then, the value of $f_t\left(\{\tildz_{it}\}_{(i,t) \notin L}; \{\tildxl_{it}\}_{(i,t) \in L}\right)$ is defined as the objective of the following LP:
\begin{align*}
\max: \quad & \sum_{(i,t) \in E} \widehat w_{it} \cdot z_{it} - \sum_{(i,t) \in L} \widehat w_{it} \cdot \tildxl_{it} & \lpsubmod \\
\text{subject to}: \quad &  \sum_{i \in U} z_{it}  ~\le~ p_t &  \\
& z_{it} ~\le~ \tildxl_{it} & \forall i:(i,t) \in L \\
& z_{it} ~\le~ \tildz_{it} & \forall i:(i,t) \notin L
\end{align*}


For simplicity, we abbreviate the notation $f_t\left(\{\tildz_{it}\}_{(i,t) \notin L}; \{\tildxl_{it}\}_{(i,t) \in L}\right)$ as $f_t(\{\tildz_{it}\})$ in the future context. Note that the value of $f_t(\{\tildz_{it}\}$ is monotone and non-negative, where the latter property is guaranteed by the observation that setting $z_{it} = \tildxl_{it}$ is a feasible solution of $\lpsubmod$. Furthermore, the following claim shows that $f_t$ is a submodular function:


\begin{Claim}
    \label{clm:submod}
    Function $f_t(\{\tildz_{it}\})$ is submodular, that is, given $\{\tildz_{it}\}$ and $\{\tildz'_{it}\}$ that satisfies $0 \leq \tildz_{it} \leq \tildz'_{it}$, for every $j: (j,t) \notin L$ and $\Delta_z \geq 0$, we have
    \[
    f_t\left(\{\tildz_{it}\}_{-j} \cup \{\tildz_{jt} + \Delta_z\}\} \right) - f_t\left(\{\tildz_{it}\} \right) ~\geq~ f_t\left(\{\tildz'_{it}\}_{-j} \cup \{\tildz'_{jt} + \Delta_z\}\} \right) - f_t\left(\{\tildz'_{it}\} \right),
    \]
    where the notations $\{\tildz_{it}\}_{-j}$ and $\{\tildz'_{it}\}_{-j}$ represents $\{\tildz_{it}\}_{i: (i,t) \notin L \land i \neq j}$ and $\{\tildz'_{it}\}_{i: (i,t) \notin L \land i \neq j}$ respectively.
\end{Claim}


Now, we show how to understand the Step $4$ of our algorithm as an online submodular welfare maximization process. Consider to view $i \in U$ as ``online items'', where the arrival order is based on the value of $t_i$\footnote{Without loss of generality, we assume each $t_i$ is unique. If there exists $i \neq i'$ such that both $i$ and $i'$ perform stage transition at the same $t$, we can add an arbitrarily small noise to both $t_i$ and $t'_i$ to make them unique, and also break the ties.}, and $t \in V$ are ``offline agents''. Note the following properties of Step $4$:

\begin{itemize}
    \item Define $\hat z^{(t)}_{it} = x^{(t_i)}_{it} \cdot \one[t \geq t_i]$. Then, for each $j \in U$, $\{x^{(t_j)}_{it}\}$ is chosen in the way that maximizes the increment of $\sum_t f_t(\{\hat z^{(t_j)}_{it}\}$, i.e., 
    \[
    \{x^{(t_j)}_{it}\} ~=~ \arg ~\max_{\{x_{it}\}} ~\sum_{t \in V} f_t\left(\{\hat z^{(t_j^-)}_{it}\}_{-j} \cup \{\hat z^{t_j}_{it} = x_{it}\}\right) - \sum_{t \in V} f_t\left( \{\hat z^{(t_j^-)}_{it}\}\right)
    \]
    subject to the constraint that $\sum_{t: (i,t) \notin L} x^{(t_j)}_{it} \leq 1 - \probfr$,
    where $t_j^{-}$ represents the time point just before vertex $j$ transitions from stage $1$ to stage $2$.
    \item For each $t \in V$, the value of $\{x^{(t)}_{is}\}$ records the optimal solution of $\lpsubmod$ that corresponds to $\hat z^{(t)}_{it}$, i.e.,
    \[
    \sum_{(i,s) \in E} \widehat w_{is} \cdot x^{(t)}_{is}  - \sum_{(i,s) \in L} \widehat w_{is} \cdot \tildxl_{is} ~=~ \sum_{s \in V} f_s(\{\hat z^{(t)}_{it}\}).
    \]
    \item The value of $f_t(\{\hat z^{(t)}_{it}\})$ is settled when online vertex $t$ arrives, because for every $i$ such that $i$ is still in stage $q$ when $t$ arrives, we have $\widehat w_{it} = 0$.
\end{itemize}


With the above observations, note that the Step $4$ in our algorithm looks similar to the greedy algorithm for online submodular welfare maximization. Therefore, the value of $\sum f_t(\{\hat z^{(t)}_{it}\}$ is at least $\frac{1}{2}$ of any other feasible solution. To be specific, we give the following lemma:

\begin{Lemma}
\label{lma:submod}
    For any $\{z_{it}\}_{(i, t) \notin L}$ such that $\sum_{t} z_{it} \leq 1 - \probfr$ is satisfied for every $i \in U$, we have
    \[
    \sum_{(i,t) \in E} \widehat w_{it} \cdot x^{(t)}_{it} - \sum_{(i,t) \in L} \widehat w_{it} \cdot \tildxl_{it} ~=~ \sum_{t \in V} f_t(\{\hat z^{(t)}_{it}\}) ~\geq~ \frac{1}{2} \sum_{t \in V} f_t(\{z_{it}\}).
    \]
\end{Lemma}
The proof of \Cref{lma:submod} is similar to the proof for the greedy algorithm of online submodular welfare maximization problem. We defer the proof of \Cref{clm:submod} and \Cref{lma:submod} to TBD.





Finally, with the help of \Cref{lem:rounding}, \Cref{lem:opt_second} and \Cref{lma:submod}, we are ready to complete the proof of Theorem~\ref{thm:lp_uniq_small}.

\begin{proof}[Proof of \Cref{thm:lp_uniq_small}]
Recall that \Cref{lem:rounding} gives
    \begin{align}
\label{eqn:alg_uniq_small}
\alg & \ge  (1-\probfr) \cdot \left( \sum_{(i,t) \in E_1} \wit \cdot x^{(t)}_{it} + \frac{1}{2} \cdot \sum_{(i,t) \in E_2} \wit \cdot x^{(t)}_{it} \right) \notag \\
& \ge (1-\probfr) \cdot \left( \sum_{(i,t) \in E_1} \wit \cdot \tildxl_{it} + \frac{1}{2} \cdot \sum_{(i,t) \in E_2 \setminus L} \wit \cdot x^{(t)}_{it} + \sum_{(i,t) \in L} \wit \cdot (x^{(t)}_{it} -\tildxl_{it}) \right) \notag \\
& \ge (1-\probfr) \cdot \left( (1-\epsalg) \cdot \lp(\tildxl) + \frac{1}{4} \cdot \lpsecond \right)~, 
\end{align}
where the first inequality holds by Lemma~\ref{lem:rounding}, the second inequality uses the fact that in stage $1$ we only collect rewards from $(i, t) \in E_1 \cap L$ and the fact that $x^{(t)}_{it} \leq \tildxl_{it}$ for $(i,t) \in E_2 \cap L$, and the last inequality holds by the the design of our algorithm and \Cref{lem:alg_free_disposal}.

It remains to lower-bound the value of $\lpsecond$. Note that the following feasible solution of program $\lpsecond$:
\[
\tildz_{it} = \begin{cases} \min(\tildxl_{it}, \yit^*) & (i,t) \in E_1  \\\yit^* & (i,t) \in E_2 \setminus L \\ 0 & (i,t) \in E_2 \cap L
\end{cases}~.
\]
Therefore, we have
\begin{align*}
\lpsecond & \ge \sum_{(i,t) \in E_2} \widehat w_{it} \cdot \tildz_{it} + \sum_{(i,t) \in E_1} \widehat w_{it} \cdot (\tildz_{it} - \tildxl_{it}) \\
& \ge \sum_{(i,t) \in E_2} \wit \cdot \yit^* - \sum_{(i,t) \in L} 2 \cdot \wit \cdot (\tildxl_{it} - \yit^*)^+ \\
&\ge 0.5 - \epsphilo - \epsu - \epsslack -4 \sqrt{\frac{\epsslack}{\epsalg}} - 2\epsslack,
\end{align*}
where the last inequality holds by Lemma~\ref{lem:opt_second} and the observation that
\[
\epsslack ~\geq~ \sum_{(i,t) \in L} w_{it} \tildxl_{it} \cdot (1 - y^*_{it}/p_t) ~\geq~ \sum_{(i,t) \in L} w_{it} \cdot (\tildxl_{it} - y^*_{it})^+.
\]
. Applying the bound on $\lpsecond$ to \eqref{eqn:alg_uniq_small}, we have 
\begin{align*}
    \alg ~&\geq~ (1-\probfr) \cdot \left( (1-\epsalg) \cdot \lp(\tildxl) + \frac{1}{4} \cdot \left( 0.5 - \epsphilo - \epsu - 3\epsslack -4 \sqrt{\frac{\epsslack}{\epsalg}} \right) \right) \\
    ~&\geq~ 0.625 - \probfr - \frac{\epsalg}{2} - \epsl - \frac{\epsphilo + \epsu + 3\epsslack}{4} - \sqrt{\frac{\epsslack}{\epsalg}}  \\
    ~&\geq~ 0.625 - 1.5 \epsslack^{1/3} - \epsphilo - \epsu - 3\epsslack,
\end{align*}
where the last inequality is satisfied when taking $\epsalg = \epsslack^{1/3}$.
\end{proof}



\subsection{Proof of \Cref{lem:rounding}}



\begin{proof}
We consider the contribution of each offline vertex $i$ to our algorithm separately.
Let $r_i = \Pr{i \text{ is matched in stage } 1}$. We first show that $r_i \le \probfr$:
\begin{align*}
r_i = \Pr{i \text{ is matched in stage }1} ~=&~ \Pr{i \text{ is proposed by some }t \le t_i} \\
=&~ 1 - \prod_{t \le t_i} (1-x^{(t)}_{it}) \le \sum_{t \le t_i} x^{(t)}_{it} \le \sum_{t \le t_i} \tildxl_{it} \le \probfr~,
\end{align*}
where we use the fact that $x^{(t)}_{it}$ is at most the initial value of $x_{it}$ when $(i,t) \in L$.
Then, the expected matching of $\ui$ from the first stage is
\begin{align*}
&\sum_{t\le t_i} \wit \cdot \Pr{\ui \text{ is proposed by } \vt } \cdot \Pr{i \text{ is unmatched before }t} \\
\ge~& \sum_{t\le t_i} \wit \cdot \Pr{\ui \text{ is proposed by } \vt } \cdot \Pr{i \text{ is unmatched at }t_i} \\
\ge~& \sum_{t\le t_i} \wit \cdot x^{(t)}_{it} \cdot (1 - \probfr) = (1-\probfr) \cdot \sum_{t: (i,t) \in E_1} \wit \cdot x^{(t)}_{it}~.
\end{align*}
Next, we consider the expected reward from the second stage. We prove by induction that every edge $(i,t)$ from the second stage (i.e., $t>t_i$) is matched with probability $\frac{1-r_i}{2}$. 
Suppose the statement holds for every $t_i < s <t$. Consider the edge $(i,t)$. According to the design of our algorithm, $(i,t)$ is selected with probability:
\begin{multline*}
\frac{1}{2 (1 - \frac{1}{2} \cdot \sum_{t_i < s < t} x^{(s)}_{is})} \cdot \Pr{\ui \text{ is proposed by } \vt } \cdot \Pr{i \text{ is unmatched before }t} \\
= \frac{1}{2 (1 - \frac{1}{2} \cdot \sum_{t_i < s < t} x^{(s)}_{is})} \cdot x^{(t)}_{it} \cdot \left(1 - r_i - \frac{1-r_i}{2} \cdot \sum_{t_i < s < t} x^{(s)}_{is} \right) = \frac{1-r_i}{2} \cdot x^{(t)}_{it}~,
\end{multline*}
where the first equation holds by induction hypothesis.
Therefore, the contribution from the second stage equals
\[
\sum_{t>t_i} \wit \cdot \frac{1-r_i}{2} \cdot \xit \ge (1-\probfr) \cdot \frac{1}{2} \cdot \sum_{t:(i,t) \in E_2} \wit \cdot \xit~.
\]
Summing the above equations over all $i \in U$ concludes the proof of the lemma.
\end{proof}



\subsection{Proof of \Cref{lem:opt_second}}

\begin{proof}
Let $U_0 \subseteq U$ be the set of vertices that the optimal algorithm matches with probability less than $\delta$, i.e.,
\[
U_0 \eqdef \left\{ \ui \in U: \sum_{t < t_i} \yit^* \le \delta \right\} \quad \text{and} \quad \overline{U_0} \eqdef U \setminus U_0~,
\]
where $\delta$ is defined to be $\sqrt{\epsslack/\epsalg}$.
Since the realization of online vertex $t$ is independent to the event that an vertex $i$ is matched before $t$, we have that
\[
\yit^* \le p_t \cdot \left( 1 - \sum_{s<t} \yit[s]^* \right), \quad \forall \ui \in U, \vt \in V~.
\]
We remark that this is the crucial constraint of previous works~\cite{} for approximating the online optimum with known arrival orders.
Applying this inequality to $t \ge t_i$, we have that
\[
\frac{\yit^*}{p_t} \le 1 - \sum_{s<t} \yit[s]^* \le 1 - \sum_{s< t_i} \yit[s]^* \le 1-\delta , \quad \forall i \in \overline{U_0}, t \ge t_i~.
\]
Furthermore, since $\{\yit^*\}$ is a feasible solution of $\lpcore$, we have that
\begin{align*}
\epsslack \ge \lpcore & \ge \sum_{i,t} \wit \cdot \tildxl_{it} \cdot \left(1 - \frac{\yit^*}{p_t} \right) + \sum_{L} \wit \cdot \yit^* \cdot \left(1 - \frac{\tildxl_{it}}{p_t} \right) \\
& \ge \sum_{i \in \overline{U_0}} \sum_{t \ge t_i} \wit \cdot \tildxl_{it} \cdot \left(1 - \frac{\yit^*}{p_t} \right) + \sum_{L} \wit \cdot \yit^* \cdot \left(1 - \frac{\tildxl_{it}}{p_t} \right) \\
& \ge \delta \cdot \epsalg \cdot \sum_{i \in \overline{U_0}} \lp_i(\tildxl) + \sum_{L} \wit \cdot (\yit^* - \tildxl_{it})^+,
% & \ge \epsalg \cdot (\delta - \probfr) \cdot \left(0.5 - \epsl \right) \cdot \lp(\overline{U_0})
\end{align*}
where the last inequality uses the fact that online vertices $t \geq t_i$ contributes at least $\epsalg$ fraction of $\lp_i(\tildxl)$. Therefore, the above inequality gives
\begin{align*}
    \sum_{i \in \overline{U_0}} \lp_i(\tildxl) ~\leq~ \frac{\epsslack}{\delta \cdot \epsalg} \qquad \text{and} \qquad \sum_{L} \wit \cdot (\yit^* - \tildxl_{it})^+ ~\leq~ \epsslack.
\end{align*}


Now, we are ready to lower-bound $\sum_{(i,t)\in E_2 \setminus L} \wit \cdot \yit^*$. We have
\begin{align}
\label{eqn:philo_second}
\sum_{(i,t)\in E_2 \setminus L} \wit \cdot \yit^* &= \philo - \sum_{(i,t)\in E_1 \cup L} \wit \cdot \yit^* \notag \\
&\ge \philo - \sum_{(i,t) \in L} \wit \cdot \yit^* - \sum_{ (i,t) \in E_1 \setminus L \land i \in U_0} \wit \cdot \yit^* - \sum_{(i,t) \in E_1 \setminus L \land i \in \overline{U_0}} \wit \cdot \yit^* 
\end{align}

It remains to bound the three summations in \eqref{eqn:philo_second} separately. For the first summation, we have
\begin{align}
    \sum_{L} \wit \cdot \yit^* ~\leq~ \sum_{L} \wit \cdot \tildxl_{it} + \sum_{L} \wit \cdot (\yit^* - \tildxl_{it})^+ ~\leq~ \lp(\tildxl) + \epsslack. \label{eq:firstsum}
\end{align}
For the second summation, we have
\begin{align}
    \sum_{ (i,t) \in E_1 \setminus L \land i \in U_0} \wit \cdot \yit^* ~\leq~ \sum_{i \in U_0} \sum_{t: (i, t) \in E_1 \setminus L} 2\lp_i(\tildx) \cdot y^*_{it} ~\leq~ 2\delta \cdot \lp(\tildx), \label{eq:secondsum}
\end{align}
where the first inequality uses the fact that $w_{it} \leq 2\lp_i(x)$ for $(i,t) \notin L$, and the second inequality uses the fact that for every $i \in U_0$, we have
\[
\sum_{t:(i,t) \in E_1 \setminus L} y^*_{it} ~\leq~ \sum_{t < t_i} y^*_{it} ~\leq~ \delta.
\]
Here, we use a critical observation that $(i, t_i) \in L$.

For the third summation in \eqref{eqn:philo_second}, we have
\begin{align}
    \sum_{(i,t) \in E_1 \setminus L \land i \in \overline{U_0}} \wit \cdot \yit^*  ~\leq~ \sum_{i \in \overline{U_0}} \sum_{t: (i, t) \in E_1 \setminus L} 2\lp_i(\tildx) \cdot y^*_{it} ~\leq~ 2\sum_{i \in \overline{U_0}} \lp_i(\tildx) ~\leq~ \frac{2\epsslack}{\delta \cdot \epsalg}, \label{eq:thirdsum}
\end{align}
where the inequality uses the fact that $w_{it} \leq 2\lp_i(x)$ for $(i,t) \notin L$. 

Finally, applying the above \eqref{eq:firstsum}, \eqref{eq:secondsum} and \eqref{eq:thirdsum} to \Cref{eqn:philo_second} together with the assumption that $\philo \geq 1 - \epsphilo$ gives
\[
\sum_{(i,t)\in E_2 \setminus L} \wit \cdot \yit^* ~\geq~ 1 - \epsphilo - \lp(\tildxl) - \epsslack - 2\delta - \frac{2\epsslack}{\delta \cdot \epsalg} ~\geq~ 0.5 - \epsphilo - \epsu - \epsslack - 4\sqrt{\frac{\epsslack}{\epsalg}},
\]
where the last inequality uses the fact that $\lp(\tildxl) \leq (0.5 + \epsu) \cdot \lp(\tildx) \leq 0.5 + \epsu$ and that $\delta := \sqrt{\epsslack/\epsalg}$.
\end{proof}
